Layout-aware Dreamer for Embodied Referring Expression Grounding

In this work, we study the problem of Embodied Referring Expression Grounding, where an agent needs to navigate in a previously unseen environment and localize a remote object described by a concise high-level natural language instruction. When facing such a situation, a human tends to imagine what the destination may look like and to explore the environment based on prior knowledge of the environmental layout, such as the fact that a bathroom is more likely to be found near a bedroom than a kitchen. We have designed an autonomous agent called Layout-aware Dreamer (LAD), including two novel modules, that is, the Layout Learner and the Goal Dreamer to mimic this cognitive decision process. The Layout Learner learns to infer the room category distribution of neighboring unexplored areas along the path for coarse layout estimation, which effectively introduces layout common sense of room-to-room transitions to our agent. To learn an effective exploration of the environment, the Goal Dreamer imagines the destination beforehand. Our agent achieves new state-of-the-art performance on the public leaderboard of the REVERIE dataset in challenging unseen test environments with improvement in navigation success (SR) by 4.02% and remote grounding success (RGS) by 3.43% compared to the previous state-of-the-art. The code is released at https://github.com/zehao-wang/LAD

==> backup/sec3-1-method.tex <==
%\subsection{Baseline Model}
=============== old version ===============

\subsubsection{Topological Graph.} 
We construct a topological graph following the work of~\citet{vlnduet}. We briefly describe the process and define the key concepts as follows.

\noindent\textbf{Graph Building.} The baseline model gradually builds a topological graph $\mathcal{G}_t = \{\boldsymbol v,\boldsymbol e \mid \boldsymbol v \subseteq \mathcal{V}, \boldsymbol e \subseteq \mathcal{E} \}$ to represent the environment at time step $t$. The graph contains three types of nodes: (1) visited nodes; (2) navigable nodes; and (3) the current node. 
%
In Fig.~\ref{fig: layout}, they are denoted by a blue circle, yellow circle and double blue circle, respectively. 
%
Both visited nodes and current node have been explored, hence the agent has access to their panoramic views, while the navigable nodes are unexplored and only partially observed by the agent from neighboring visited nodes. At each step $t$, we build the graph $\mathcal{G}_t$ by updating the current node $a_{t,0}$ and its neighbouring 
%unvisited navigable nodes $\mathcal{N}(V_t)$ to $\mathcal{G}_{t-1}$. 
navigable nodes $\mathcal{A}_t$. 
%Figure [] illustrates this process.

\noindent\textbf{Node Representation.} When navigating to a node $a_{t,0}$ at time step $t$, the agent extracts panoramic image features $\mathcal{R}_t$ and object features $\mathcal{O}_t$ from its panoramic view $\mathcal{V}_t$. Bounding boxes of objects are obtained by an object detection model~\cite{anderson2018bottom} or directly provided by simulation environment, as is the case in the REVERIE dataset.
Since current node is fully observed at this stage, we update its features by more informative local visual features. Specifically, we implement a multi-layer transformer with self-attention among the image features $\mathcal{R}_t$ and object features $\mathcal{O}_t$ observed at the current location to model their relations. The fused features $\hat{\mathcal{O}_t}$ and $\hat{\mathcal{R}_t}$ are treated as local visual features of node $a_{t,0}$.
%
Then we update the representations of nodes in topological graph as follows: (1) For the current node, we concatenate and average pool the local features $\hat{\mathcal{R}_t}$ and $\hat{\mathcal{O}_t}$ to update its representation;
%
(2) As unvisited nodes could be partially observed from different directions of multiple visited nodes, we average all image features of the partial views as its representation.
%(3) The initial features before graph attention module of previously visited nodes will be kept unchanged.
(3) The representation of previously visited node remains unchanged.
%
We then further add the location embedding and navigation step embedding to the representation of each node. The location embedding of a node if formed by the concatenation of Euclidean distance, heading and elevation angles relative to the current node, and similar to positional embeddings the step embedding embeds the last visited time step of each visited node and we set time step zero for unvisited nodes. We use $\mathcal{H}_t$, %$\mathcal{H}_{t}^{\spadesuit}$, $\mathcal{H}_t^{\heartsuit}$ 
to denote the full node representation. Please refer to Appendix for further details.

%visited node representation and unvisited node representation of current topological graph $\mathcal{G}_{t}$, respectively: 


% \begin{align*}
%     \mathcal{H}_{t} = \{\mathcal{H}_{t}^{\spadesuit}, \mathcal{H}_t^{\heartsuit} \} \tag{1}
% \end{align*}










==> backup/sec3-2-method.tex <==
%\subsection{Global Visual and Cross Model Attention}
\noindent\textbf{Language Encoder.} We use a pretrained multi-layer transformer encoder~\cite{transformer} to encode the natural language instruction $\mathcal{X}$. Following the convention, we feed the sum of the token embedding, position embedding and token type embedding into the transformer encoder, and the output denoted as $\mathcal{T}$ is taken as language features.

\noindent\textbf{Global Node Self-Attention.} To enable that each node perceives global environment information and can be further used to learn room-to-room correlations in the environment layout, we conduct a graph aware self attention (GASA) \cite{vlnduet} over node embeddings $\mathcal{H}_t$ of graph $\mathcal{G}_t$. For simplicity, we use the same symbol $\mathcal{H}_t$ to denote the encoded graph node embeddings.

%\begin{align*}
%    \mathcal{H}'_t &= Softmax(\frac{\mathcal{H}_tW_q(\mathcal{H}_tW_k)^T}{\sqrt{d}} + M)\mathcal{H}_tW_v \tag{1}  \\ 
%    M &= \mathcal{D}W_e + b_e  \tag{2}\\
%\end{align*}
%where $W_{q,k,v,e}$ are learnable parameters, $\mathcal{H}_t$ denotes node representation of nodes at time step $t$, and $\mathcal{D}$ is the pair-wise distance matrix of graph $\mathcal{G}_t$.


\noindent\textbf{Cross Graph Language Encoder.} We use a cross modal transformer~\cite{lu2019vilbert} to model both the global and local graph-language relation. We name the global and local graph-language co-attention models as global branch and local branch, respectively. For the global branch, we perform co-attention of node embeddings $\mathcal{H}_t$ over language features $\mathcal{T}$, while only the current node and its neighbouring navigable nodes are used to compute the co-attention in the local branch. We feed the outputs of the global branch to the \text{Layout Learner} for layout prediction. In addition, the local branch outputs a predicted action distribution and score for object grounding, while the global branch only generates an action distribution. The action predictions from global and local branches are fused to make final decision Fig.~\ref{fig: layout}.

%both the global and local branch outputs are further used to make the navigation decision at current time step $t$ as shown in Fig.~\ref{fig: layout}. Meanwhile the local branch also

\begin{align*}
    \mathcal{\tilde{H}}_t^{(glo)} &= \text{Cross-Attn}(\mathcal{H}_t, \mathcal{T}, \mathcal{T})  \tag{1} \\
    \mathcal{\tilde{H}}_t^{(loc)} &= \text{Cross-Attn}(\{\mathcal{H}_t(\mathcal{A}_t), \mathcal{H}_t(a_{t,0})\}, \mathcal{T}, \mathcal{T}) \tag{2}
\end{align*}
where \textit{$\text{Cross-Attn}(query, key, value)$} is a multi-layer transformer decoder, and $\mathcal{A}_t$ stands for neighbouring navigable nodes of the current node $a_{t,0}$. $\mathcal{H}_t(\cdot)$ represents extracting corresponding rows from $\mathcal{H}_t$ by node indices.








